Exploiting Social Navigation

We present an effective Sybil attack against social location based services. Our attack is based on creating a large number of reputed "bot drivers", and controlling their reported locations using fake GPS reports. We show how this attack can be used to influence social navigation systems by applying it to Waze - a prominent social navigation application used by over 50 million drivers. We show that our attack can fake traffic jams and dramatically influence routing decisions. We present several techniques for preventing the attack, and show that effective mitigation likely requires the use of additional carrier information.

==> abstract2.tex <==
\begin{abstract}
We present an effective Sybil attack~\cite{DBLP:conf/iptps/Douceur02} against social navigation services. Our attack is based on creating a large number of reputed ``bot drivers'', and using fake GPS reports to move ``bot drivers'' according to desired traffic patterns.
We show how this attack can be used to influence social navigation systems by applying it to ``Waze''~\cite{Waze} - a prominent social navigation application used by over $50$ million drivers. We show that our attack can fake traffic jams and dramatically influence routing decisions. We present several techniques for preventing the attack, and show that effective mitigation likely requires the use of additional carrier information.
\end{abstract}


==> intro.tex <==
\section{Introduction}

Social navigation is rapidly becoming a prevalent approach for navigation. The Waze social navigation application collects navigation data such as route duration, traffic congestion, road obstacles, and even map layout from users, and then uses this information to route other users.

With a community of $50$ million users~\cite{GoogleBoughtWaze}, social navigation data is becoming a \emph{reliable} source of navigation information trusted by many. For example, Waze traffic information is used to feed reports for various Radio and TV stations~\cite{WazeOnTV}, as well as the widely used Google Maps navigation application. This propagates the influence of social navigation to a much wider community.

In this paper, we present the first Sybil attack on social navigation systems. In a Sybil attack the attacker subverts the reputation system of a network by creating a large number of pseudonymous identities, using them to gain a disproportionately large influence~\cite{DBLP:conf/iptps/Douceur02}. Our attack is cheap and could be facilitated using mostly off-the-shelf components. We demonstrate the effectiveness of our attack by applying it to Waze, the popular social navigation system (recently acquired by Google~\cite{GoogleBoughtWaze}). We show that our technique can be used to simulate traffic jams, and dramatically influence the routing decisions presented to users.

\paragraph{Main Contributions} The main contributions of this paper are:
\begin{itemize}
\item We present the first Sybil attack on social navigation systems.
\item Our attack is inexpensive and can be facilitated using mostly off-the-shelf emulation software, a simple mock GPS application, and the Android Debug Bridge.
\item We demonstrate our approach by simulating traffic jams, and affecting the routing presented to drivers.
\item We present two approaches for mitigating our attack and similar attacks on social navigation: using carrier information and user behavioral analysis. We evaluate them based on parameters of simplicity, user experience, effectiveness and cost.
\end{itemize}

